Towards Stronger Blockchains: Security Against Front-Running Attacks

Blockchains add transactions to a distributed shared ledger by arriving at consensus on sets of transactions contained in blocks. This provides a total ordering on a set of global transactions. However, total ordering is not enough to satisfy application semantics under the Byzantine fault model. This is due to the fact that malicious miners and clients can collaborate to add their own transactions ahead of correct clients' transactions in order to gain application level and financial advantages. These attacks fall under the umbrella of front-running attacks. Therefore, total ordering is not strong enough to preserve application semantics. In this paper, we propose causality preserving total order as a solution to this problem. The resulting Blockchains will be stronger than traditional consensus based blockchains and will provide enhanced security ensuring correct application semantics in a Byzantine setting.

==> 10-asf.tex <==

\begin{section}{Application Semantics Forking Attack}



Forking attacks \cite{wang2019corking} have been studied extensively to formally analyze the security characteristics of blockchain. A forking attack typically aims to create a fork in the blockchain with the intention of carrying out a double-spending attack. In this paper, we present a variant of the classic forking attack which we call the \textit{application semantics forking attack} (ASF attack).
To the best of our knowledge such an attack has not been carried out or studied in the literature. An ASF attack aims to create a fork in the blockchain with the intention of disturbing the application semantics of a decentralized application. The motivation for a miner or a set of miners here may not necessarily be financial, but instead based on a variety of real-world factors. 

Consider a decentralized social network on the blockchain. Honest processes send messages to a particular social media thread in the form of transactions. A malicious miner can destroy application semantics by executing the following steps:

\begin{enumerate}
    \item 
\end{enumerate}

\begin{definition}
    \label{def:asf}

    \textbf{ASF Attack}
    
\end{definition}

\begin{lemma}
    \label{lm:semantics1}
    A miner that attempts to transform a valid blockchain to a forked blockchain is Byzantine.
   
\end{lemma}


\begin{lemma}
    \label{lm:semantics2}
    Application semantics are captured by the happens before relation.
\end{lemma}

\begin{theorem}

\label{th:semantics}

ASF attacks require violation of causal ordering across transactions.

\end{theorem}

\begin{corollary}
    \label{c:asf}
    ASF attacks are a subset of causal ordering violation attacks.
\end{corollary}

\end{section}

